Representation Learning for Online and Offline RL in Low-rank MDPs

This work studies the question of Representation Learning in RL: how can we learn a compact low-dimensional representation such that on top of the representation we can perform RL procedures such as exploration and exploitation, in a sample efficient manner. We focus on the low-rank Markov Decision Processes (MDPs) where the transition dynamics correspond to a low-rank transition matrix. Unlike prior works that assume the representation is known (e.g., linear MDPs), here we need to learn the representation for the low-rank MDP. We study both the online RL and offline RL settings. For the online setting, operating with the same computational oracles used in FLAMBE (Agarwal et.al), the state-of-art algorithm for learning representations in low-rank MDPs, we propose an algorithm REP-UCB Upper Confidence Bound driven Representation learning for RL), which significantly improves the sample complexity from $\widetilde{O}( A^9 d^7 / (\epsilon^{10} (1-\gamma)^{22}))$ for FLAMBE to $\widetilde{O}( A^2 d^4 / (\epsilon^2 (1-\gamma)^{5}) )$ with $d$ being the rank of the transition matrix (or dimension of the ground truth representation), $A$ being the number of actions, and $\gamma$ being the discounted factor. Notably, REP-UCB is simpler than FLAMBE, as it directly balances the interplay between representation learning, exploration, and exploitation, while FLAMBE is an explore-then-commit style approach and has to perform reward-free exploration step-by-step forward in time. For the offline RL setting, we develop an algorithm that leverages pessimism to learn under a partial coverage condition: our algorithm is able to compete against any policy as long as it is covered by the offline distribution.

==> computationally_efficient.tex <==
\section{Computationally efficient version}

\begin{lemma}[Finite horizon performance difference lemma]

\begin{align*}
    V^{\pi}_{P,r}(d_0)- \E_{s_0\sim d_0}[f_0(s_0,\pi)]=\sum_t \gamma^t \E_{(s,a)\sim d^{\pi}_{P,t}}[r(s,a) +\gamma \EE_{s'\sim P(s'\mid s,a)}[f_{t+1}(s',\pi)]-f_t(s,a)] ]. 
\end{align*}
\end{lemma}

\masa{not yet}


\begin{algorithm}[!htp]
\caption{------ }
\begin{algorithmic}[1]
  \STATE {\bf  Input:} Regularizer $\lambda$, Model classes $\Mcal=\{\mu^{\top}\phi:\mu\in \Psi,\phi\in \Phi\}$, Dataset $\Dcal$, Reward $r'(s,a)$
  \STATE Learn a model $\hat P $ by MLE: $\hat P=\hat \mu^{\top}\hat \phi=\argmax_{P\in \Mcal}\E_{\Dcal}[\ln P(s'\mid s,a)]$.
  \STATE Set some $H,\hat \theta_{H+1}=0$. 
  \FORALL{$t=H,\cdots,0$}
 \STATE 
 \begin{align*}
      \hat \theta_t=\argmin_{\theta \in \Theta_t}\E_{\Dcal}[\{\gamma \hat V_{t+1}(s')-\theta^{\top}_t\hat \phi(s,a)\}^2]
 \end{align*}
 \STATE  $\hat Q_t(s,a)= r'(s,a)-b'(s,a)+\hat \theta^{\top}_t\hat \phi(s,a)$, $\hat V_t(s)=\hat Q_t(s,\pi)$. 
 \ENDFOR 
 \STATE Output $\hat \theta_0$
\end{algorithmic}
\end{algorithm}

Here, $r'=r-b$. Remark $r-b$ is not linear in $\phi$ and lie in $[-1/(1-\gamma)^2,1/(1-\gamma)^2]$. This leads to the above regression way. 
And $\hat V_0=\hat Q_0(s_0,\pi)$. we want to show $V^{\pi}_{\hat P,r'}(d_0)- \hat V_0(d_0)\geq c_1$ for some $c_1$.  

\begin{align*}
  & V^{\pi}_{\hat P,r'}(d_0)- \hat V_0(d_0)\\
  &=\sum_{t=0}^{\infty} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[ r'(s,a)+\gamma  \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')]-\hat Q_{t}(s,a)] \tag{Performance difference lemma}\\
  &=\sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[r'(s,a)+\gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')]  -\hat Q_{t}(s,a)]+\\
  &+\sum_{t=H+1}^{\infty} \gamma^t  \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[r'(s,a)+\gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')]  -\hat Q_{t}(s,a)]\\
   &\geq \sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[r'(s,a)+\gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')]  -\hat Q_{t}(s,a)] -\frac{\gamma^{H+1}}{1-\gamma}\|r'(s,a)\|_{\infty}. 
\end{align*}
Then, 
\begin{align*}
&\sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[r'(s,a)+\gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')]  -\hat Q_{t}(s,a)]\\
&=\sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[ b'(s,a)+\gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')]  -\hat \theta^{\top}_t \hat \phi_t(s,a)]\\
&=\sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[ b'(s,a)+\underbrace{\gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')]  -\gamma \EE_{s'\sim P^{\star}(s'\mid s,a)}[\hat V_{t+1}(s')]}_{(a)}] ]\\
&+\sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[\underbrace{\gamma \EE_{s'\sim P^{\star}(s'\mid s,a)}[\hat V_{t+1}(s')]  - \hat \theta^{\top}_t \hat \phi_t(s,a)}_{(b)}] 
\end{align*}
We use the following fact: for any $g_t:\Scal \times \Acal \to \RR$, we have 
\begin{align*}
    &\sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{t}}[g_t(s,a)]\\
    &\leq \E_{(s,a)\sim d^{\pi}_{0}}[g_0(s,a)]+   \sum_{t=0}^{H-1} \gamma^{t+1} \E_{(s,a)\sim d^{\pi}_{\hat P,{t}}}[\|\hat \phi(s,a)\|_{\Sigma^{-1}_{\rho,\hat \phi}}]\sqrt{n\omega \E_{\rho}[g^2_{t+1}(s,a)]+\lambda d\|g_{t+1}\|^2_{\infty}+ n\zeta   }. 
\end{align*}

We denote the term (b) as $g'_t$. Here, we want to substitute $g_t$ with $g'_t$. 
\begin{align*} 
    \E_{\rho}[g'^2_t(s,a)]\leq \min_{\|\theta\|_2\leq \Theta_t}\E_{(s,a)\sim \rho}[ \{ \gamma \EE_{s'\sim P^{\star}(s'\mid s,a)}[\hat V_{t+1}(s')]- \theta^{\top}\hat \phi(s,a) \}^2]+\mathrm{Error}
\end{align*}
where $\mathrm{Error}=o(c/N)$.

Noting \masa{I suppose $b'\leq (1-\gamma)^{-2}$}
\begin{align*}
   & \|\hat Q_t\|_{\infty}\leq \|r'\|_{\infty}+\|b'\|_{\infty}+\|\hat \theta^{\top}_t\hat \phi\|_{\infty}\leq \frac{1}{1-\gamma}+\|\hat \theta_t\|_2 =(1-\gamma)^{-2}+\Theta_t \\ 
   &\left \|\gamma  \int \hat V_{t+1}(s')\mu^{\top}(s')\rd(s')\right\|_2\lesssim \prns{\gamma (1-\gamma)^{-2}+\gamma \Theta_{t+1}}\sqrt{d}=\Theta_t.
\end{align*}
\masa{this is an issue. leads to an exponential blowup in $d$. We need to ensure $\|\hat V_t\|_{\infty}$ is bounded by some constant independent of $t$}
this is further decomposed as 
\begin{align*}
    \E_{\rho}[g'^2_t(s,a)]&\leq \E_{(s,a)\sim \rho}\left[ \{ \gamma \EE_{s'\sim P^{\star}(s'\mid s,a)}[\hat V_{t+1}(s')]-  \gamma  \int \hat V_{t+1}(s')\mu^{\top}(s')\rd(s')  \hat \phi(s,a) \}^2\right]+\mathrm{Error}\\
    &\leq \E_{(s,a)\sim \rho}\left[ \{ \gamma \EE_{s'\sim P^{\star}(s'\mid s,a)}[\hat V_{t+1}(s')]- \gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')] \}^2\right]+\mathrm{Error} \\ 
    &\leq \gamma^2\|\hat V_{t+1}\|^2_{\infty} \E_{(s,a)\sim \rho}\left[ \|\hat P(\cdot \mid s,a)- P^{\star}(\cdot \mid s,a)\|^2_2\right]+\mathrm{Error}. 
\end{align*}

We denote the term (a) as $g"_t$.\masa{this term is fine. }

---------------------------


One way to avoid is as follows. \masa{Ensure something like $\|\hat V_t\|_{\infty}\leq (1-\gamma)^{-2}$ by truncation and set $\Theta_t=(1-\gamma)^{-2}\sqrt{d }$. }


\begin{algorithm}[!htbp]
\caption{------ }
\begin{algorithmic}[1]
  \STATE {\bf  Input:} Regularizer $\lambda$, Model classes $\Mcal=\{\mu^{\top}\phi:\mu\in \Psi,\phi\in \Phi\}$, Dataset $\Dcal$, Reward $r'(s,a)$
  \STATE Learn a model $\hat P $ by MLE: $\hat P=\hat \mu^{\top}\hat \phi=\argmax_{P\in \Mcal}\E_{\Dcal}[\ln P(s'\mid s,a)]$.
  \STATE Set some $H,\hat \theta_{H+1}=0$. 
  \FORALL{$t=H,\cdots,0$}
 \STATE 
 \begin{align*}
      \hat \theta_t=\argmin_{\theta \in \Theta_t}\E_{\Dcal}[\{\gamma \hat V_{t+1}(s')-\theta^{\top}_t\hat \phi(s,a)\}^2]
 \end{align*}
 \STATE  $\hat Q_t(s,a)= r'(s,a)-b'(s,a)+\max(\min(\hat \theta^{\top}_t\hat \phi(s,a),1/(1-\gamma)^3),-1/(1-\gamma)^3)$
 \STATE $\hat V_t(s)=\hat Q_t(s,\pi)$. 
 \ENDFOR 
 \STATE Output $\hat \theta_0$
\end{algorithmic}
\end{algorithm}

Then, we would have 
\begin{align*}
   & V^{\pi}_{\hat P,r'}(d_0)- \hat V_0(d_0)\\
   &\geq \sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[r'(s,a)+\gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')] -\hat Q_t(s,a)]\\
   &=\sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[b'(s,a)+\gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')] - \max(\min(\hat \theta^{\top}_t\hat \phi(s,a),1/(1-\gamma)^3),-1/(1-\gamma)^3) ]\\
   &\geq \sum_{t=0}^{H} \gamma^t \E_{(s,a)\sim d^{\pi}_{\hat P,t}}[b'(s,a)+\gamma \EE_{s'\sim \hat P(s'\mid s,a)}[\hat V_{t+1}(s')] - \max(\hat \theta^{\top}_t\hat \phi(s,a),-1/(1-\gamma)^3) ]\\
\end{align*}
.......................


==> preliminary.tex <==
\section{Preliminaries}
\label{sec:prelim}
We consider an episodic discounted infinite horizon Markov Decision Process $\Mcal=\langle \Scal,\Acal,P,r,\gamma,d_0\rangle $ specified by a state space $\Scal$, a discrete action space $\Acal$, a transition model $P:\Scal\times \Acal\to \Delta(\Scal)$, a reward function $r:\Scal \times \Acal \to \mathbb{R}$, a discount factor $\gamma\in [0,1)$, and an initial distribution $d_0\in \Delta(\Scal)$. To simplify the presentation, we assume $r(s,a)$ and $d_0$ are known (e.g., when $d_0$ is a probability mass only on $s_0$, agent always starts from a fixed initial state $s_0$)\footnote{Extension to the unknown case is straightforward. Recall the major challenging of RL is due to the unknown transition model.}. Following prior work \citep{jiang2017contextual,sun2019model}, we assume \emph{trajectory reward is normalized}, i.e., for any trajectory $\{s_h,a_h\}_{h=0}^{\infty}$, we have $\sum_{h=0}^{\infty} \gamma^h r(s_h,a_h) \in [0,1]$. Since the ground truth $P^{\star}$ is unknown, we need to learn it by interacting with environments in an online manner or utilizing offline data at hand.  We remark that the extension of our all results  to the finite horizon nonstationary case is straightforward. %

\begin{wrapfigure}{r}{0.34\textwidth}
\vspace{-20pt}
  \begin{center}
    \includegraphics[width=0.34\textwidth]{latent_rep}
  \end{center}
  \vspace{-10pt}
  \caption{A latent state model captured by low-rank MDP. Here $\phi^\star(s,a)$ is a distribution over a discrete latent state space $\mathcal{Z}$. Note that this is still a Markovian model as there is no transition among latent states.}
  \vspace{-10pt}
  \label{fig:latent_rep}
\end{wrapfigure}

We use the following notation. Given a policy $\pi:\Scal \to \Delta(\Acal)$, which maps from state to distribution over actions and some model $P$, we define the value function $V^{\pi}_{P}(s) = \mathbb{E}\left[ \sum_{h=0}^{\infty} \gamma^h r(s_h,a_h) | s_0 = s, P, \pi \right]$ to represent the expected total discounted reward of $\pi$ under $P$ starting at $s$. Similarly, we define the state-action Q function $Q^{\pi}_P(s,a) := r(s,a) + \gamma \EE_{s'\sim P(\cdot | s,a)} V^{\pi}_P(s')$. The expected total discounted reward of a policy $\pi$ under transition $P$ and reward $r$ is denoted as $V^{\pi}_{P,r} := \EE_{s_0\sim d_0} V^{\pi}_P(s_0)$.
We define the discounted state-action occupancy distribution $d^{\pi}_P(s,a)=(1-\gamma)\sum_{t=0}^{\infty} \gamma^t d^{\pi}_{P,t}(s,a)$, where $d^{\pi}_{P,t}(s,a)$ is the probability of $\pi$ visiting $(s,a)$ at time step $t$ under $\pi$ and $P$. We slightly abuse the notation, and denote $d^{\pi}_{P}(s)$ as the state visitation, which is  equal to $\sum_{a\in\Acal} d^{\pi}_P(s,a)$. When $P$ is the ground truth transition model $P^\star$, we drop the subscript and simply use $d^{\pi}$ to denote its state-action distribution. Unless otherwise noted, $\Pi$ denotes the class of all polices $\{S\to \Delta(\Acal)\}$. We denote total variation distance of $P_1$ and $P_2$ by $\|P_1-P_2\|_1$. Finally, given a vector $a$, we define $\|a\|_2=\sqrt{a^{\top}a},\|a\|_{B}=\sqrt{a^{\top}Ba}$. $c_0,c_1,\cdots$ are universal constants. 



We study low-rank MDPs defined as follows \citep{jiang2017contextual,Agarwal2020_flambe}. The conditions on the upper bounds of the norm of $\phi^{\star},\mu^{\star}$ are just for normalization.   
\begin{definition}[Low-rank MDP]
A transition model $P^{\star}:\Scal\times \Acal \to \Delta(\Acal)$ admits a low rank decomposition with rank $d\in \NN$
if there exists two embedding functions $\phi^{\star}\, \mu^{\star}$ such that 
\begin{align*}
    \forall s,s'\in \Scal, a\in \Acal: P^{\star}(s'\mid s,a)=\mu^{\star}(s')^{\top}{\phi^{\star}(s,a)}
\end{align*}
where $\|\phi^{*}(s,a)\|_2\leq 1$ for all $(s,a)$ and for any function $g:\Scal \to [0,1]$, $\|\int \mu^{\star}(s)g(s)\rd(s)\|_2\leq \sqrt{d}$. An MDP is a low rank MDP if $P^{\star}$ admits such a low rank decomposition.  
\end{definition}

Low-rank MDPs capture the latent variable model \citep{Agarwal2020_flambe} shown in \pref{fig:latent_rep} where $\phi^\star(s,a)$ is a distribution over a discrete latent state space $\mathcal{Z}$. The block-MDP model \citep{du2019provably} is a special  instance of the latent variable model with $\phi^\star(s,a)$ being a one-hot encoding vector. 
Note the linear MDPs \citep{YangLinF2019RLiF,jin2020provably} assume $\phi^\star$ is known.  %




Next, we explain two settings: the online learning setting and the offline learning setting. Then, we present our function approximation setup and computational oracles. 

\vspace{-0.1cm}
\paragraph{Episodic Online learning}
In online learning, our overall goal is  to learn a stationary policy $\hat \pi$ so that it maximizes $V^{\hat \pi}_{P^{\star},r}$, where $P^\star$ is the ground truth transition.  We assume that we operate under the episodic learning setting where we can only reset to states sampled from the initial distribution $d_0$ (e.g., to emphasize the  challenge from exploration, we can consider the special case where we can only reset to a fixed $s_0$). In the episodic setting, given a policy $\pi$, sampling a state $s$ from the state visitation $d_P^{\pi}$ is done by the following \emph{roll-in} procedure: starting at $s_0\sim d_{0}$, at every time step $t$, we terminate and return $s_t$ with probability $1-\gamma$, and otherwise we execute $a_t\sim \pi(s_t)$ and move to $t+1$, i.e., $s_{t+1} \sim P(\cdot | s_t,a_t)$. Such a sampling procedure is widely used in the policy gradient and policy optimization literature (e.g., \citep{kakade2002approximately,agarwal2021theory,agarwal2020pc}). 
\looseness=-1 %





\vspace{-0.1cm}
\paragraph{Offline learning} In the offline RL, we are given a static dataset in the form of quadruples:
\begin{align*}\textstyle
    \Dcal=\{s^{(i)}, a^{(i)}, r^{(i)}, s'^{(i)}\}_{i=1}^n\sim \rho(s,a)\delta(r=r(s,a))P^{\star}(s'\mid s,a). 
\end{align*} 
For simplicity, we assume $\rho=d^{\pi_b}_{P^{\star}}$, where $\pi_b \in \Scal\to \Delta(\Acal)$ is a fixed behavior policy. We  denote $\EE_{\Dcal}[f(s,a,s')]=1/n\sum_{(s,a,s')\in \Dcal}f(s,a,s')$. To succeed in offline RL, we in general need some coverage property of $\rho$. One common assumption is that $\rho$ globally covers every possible policies' state-action distribution, i.e., $\max_{\pi,s,a}d^{\pi}_{P^\star}(s,a) / \rho(s,a) < \infty$ \citep{antos2008learning}. In this work, we relax such a global coverage assumption and work under the \emph{partial} coverage condition where $\rho$ may not cover distributions of all possible policies. Instead of competing against the optimal policy under the global coverage, we aim to compete against any policies covered by the offline data. %
In section~\ref{sec:offline}, we will precisely define the partial coverage condition using the concept of the relative condition number \citep{agarwal2021theory}. %
\looseness=-1







\vspace{-0.1cm}
\paragraph{Function approximation setup and computational oracles} 

Since $\mu^\star$ and $\phi^\star$ are unknown, we use function classes to capture them. Our function approximation and computational oracles are \emph{exactly the same as the ones used in \flambe}. For completeness, we state the function approximation and computational oracles below.  %

\begin{assum}\label{assum:basic}
We have a model class $\Mcal = \{ (\mu, \phi): \mu\in \Phi, \phi\in\Phi \}$, where $\mu^\star\in \Phi$, $\phi^\star\in\Phi$.%
\end{assum} 
Following the norm bounds on $\mu^\star, \phi^\star$  we similarly assume that the same norm bounds hold for our function approximator, i.e., for any $\mu\in \Phi,\phi\in \Phi$, $\|\phi(s,a)\|_{2} \leq 1$, 
$\forall (s,a)$ and $\|\int \mu(s)g(s)\rd(s)\|_2\leq \sqrt{d},\forall g:\Scal \to [0,1]$, and $\int \mu^{\top}(s')\phi(s,a)\rd(s')=1,\,\forall (s,a)$. \looseness=-1

As  for computational oracles, we use  a supervised learning style MLE oracle. 
\begin{definition}[Maximum Likelihood Oracle (MLE)] \label{asm:mle}
Consider the model class $\Mcal$ and a dataset $\mathcal{D}$ in the form of $(s,a,s')$, the MLE oracle returns the maixmum likelihood estimator $\hat P := (\hat\mu,\hat\phi) = \argmax_{(\mu,\phi)\in\Mcal} \EE_{\Dcal} \ln (\mu(s')^{\top}\phi(s,a))$.
\end{definition}
We also invoke a planning procedure for \emph{known linear MDPs with potentially nonlinear rewards}, which can be done in polynomial time (after all, we know that online learning in linear MDPs can be done statistically and computationally efficient). 
Given a reward $r$ and a model $P:= (\mu,\phi)$ with $P(s' | s,a) = \mu(s')^{\top} \phi(s,a)$ (i.e., a \emph{known linear transition} with a \emph{known} feature $\phi$), we can compute the optimal policy $\arg\max_{\pi} V^{\pi}_{P,r}$ by standard least square value iteration which uses linear regression. 
A planning procedure for a known linear MDP is also used in \flambe, see Section 5.1 in \citet{Agarwal2020_flambe} for details of how to implement this procedure for a known linear MDP with polynomial computation complexity.   \looseness=-1





==> something_old.tex <==


Consider a finite horizon MDP $\Mcal=\langle \Scal,\Acal,d_0,P^{\star} \rangle $. Given a policy $\pi_i$ at episode $i$, we have online data:
\begin{align*}
   \Dcal'_{i} &=\{s^i,a^i\}\sim  d^{\pi"_i}(a,s),\,  d^{\pi"_i}(s,a)=1/(H+1) \sum_{j=0}^{H}  d^{\pi"_i}_{j},\,d^{\pi"_i}_{j}(a,s)=d^{\pi_i}_{j,P^{\star}}(s)u(a|s), 
\end{align*}
where $u(a\mid s)$ is an uniform distribution and $d^{\pi_i}_{j,P^{\star}}(s)$ is a marginal state distribution following $\pi_i$ at $j$. We also define
\begin{align*}
    \rho_i=\frac{1}{i-1} \sum_{j=1}^{i-1} d^{\pi"_j},\quad  d^{\pi_i}_{P^{\star}}=\frac{1}{H} \sum_{j=1}^{H} d^{\pi_i}_{j,P^{\star}}. 
\end{align*}

Then, define $   \Dcal_{i}= \{\Dcal'_{j}\}_{j=1}^{i-1} $. Basically, $\Dcal_i\sim \rho_i$. 
We consider the following naive method. 
\begin{enumerate}
    \item Using $ \Dcal_{i}$, learn 
    \begin{align*}
        \hat P_i=(\hat \mu_i,\hat \phi_i)=\argmax_{\mu \in \Psi, \phi \in \Phi }\EE_{\Dcal_i}[\ln(\mu(s)^{\top}\phi(s,a))]. 
    \end{align*}
    \item Using $ \Dcal_{i}$, set the bonus:  
    \begin{align*}
        \hat b_i(s,a)=\alpha \sqrt{\hat \phi_i(s,a)^{\top}\hat \Sigma^{-1}_{i}\hat \phi_i(s,a)}, \hat \Sigma_{i}=\sum_{j=1}^{i-1}\hat \phi_i(s^j,a^j)\hat \phi_i^{\top}(s^j,a^j)+\lambda I. 
    \end{align*}
    \item Solve $\pi_i=\argmax_{\pi}V^{\pi}_{\hat P_i,r+\hat b_i}$. 
\end{enumerate}

\begin{lemma}
Consider an episode $i$.  Then, 
\begin{align*}
    \alpha = H\sqrt{\frac{|\Acal|i}{\gamma}\zeta + 4\lambda d+i \zeta},\quad \lambda=O(d\log (|\Phi||\Psi|n/\delta)),\zeta=O(\log(|\Phi||\Psi|n/\delta)/i). 
\end{align*}
With probability $1-\delta$, 
\begin{align*}
    \forall \pi \in \Pi, V^{\pi}_{\hat P_i,r+\hat b_i}- V^{\pi}_{P^{\star}}\geq -\frac{1-\gamma}{\gamma}|\Acal|\zeta. 
\end{align*}
\end{lemma}
Roughly, $\alpha=(1-\gamma)^{-1}\sqrt{d^2\ln(|\Phi||\Psi|n/\delta)}$. 

\begin{proof}
We define 
\begin{align*}
    \rho_i &=\frac{1}{(i-1)}\sum_{j=1}^{i-1} d^{\pi"_j}(s,a), \, d^{\pi"_i}(s,a)=\frac{1}{H}\sum_{t=0}^{H-1} d^{\pi"_i}_t(s,a),\,
    \Sigma_{\rho_i,\phi}=(i-1)\EE_{(s,a)\sim \rho_i}[\phi\phi^{\top}] +\lambda I,\\
     \rho^{(1)}_i &=\frac{1}{(i-1)}\sum_{j=1}^{i-1} d^{\pi"_j}(s,a),  d^{\pi"_i}(s,a)=\frac{1}{H+1}\sum_{t=1}^H d^{\pi"_i}_t(s,a),\,
    \Sigma_{\rho_i,\phi}=(i-1)\EE_{(s,a)\sim \rho_i}[\phi\phi^{\top}] +\lambda I,\\
     \rho^{(2)}_i &=\frac{1}{(i-1)}\sum_{j=1}^{i-1} d^{\pi"_j}(s,a),  d^{\pi"_i}(s,a)=\frac{1}{H+2}\sum_{t=1}^{H+1} d^{\pi"_i}_t(s,a),\,
    \Sigma_{\rho_i,\phi}=(i-1)\EE_{(s,a)\sim \rho_i}[\phi\phi^{\top}] +\lambda I. 
\end{align*}
From performance difference lemma, 
\begin{align*}
    V^{\pi}_{\hat P_i,r+\hat b_i}- V^{\pi}&=H\EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\bracks{\hat b_i(s,a)+\EE_{s'\sim \hat P_i(s,a)}\bracks{V^{\pi}(s') } - \EE_{s'\sim P^{\star}(s,a)}\bracks{V^{\pi}(s') } }\\
    &\geq H\EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\bracks{\alpha \|\hat \phi_i(s,a)\|_{ \Sigma^{-1}_{\rho^{(1)}_i,\hat \phi_i}}+\EE_{s'\sim \hat P_i(s,a)}\bracks{V^{\pi}(s') } - \EE_{s'\sim P^{\star}(s,a)}\bracks{V^{\pi}(s') } } \tag{from \pref{lem:con}}. 
\end{align*}
Here, by letting $f(s,a)=\|\hat P_i(\cdot \mid s,a)-P^{\star}(\cdot \mid s,a)\|_1$, we have 
\begin{align*}
   |\EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\braces{\EE_{s'\sim \hat P_i(s,a)}\bracks{V^{\pi}(s') } - \EE_{s'\sim P^{\star}(s,a)}\bracks{V^{\pi}(s') }}|\leq H\EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\braces{f(s,a)}. 
\end{align*}
Besides, we have 
\begin{align}\label{eq:first}
    \EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\braces{f(s,a)}\leq  \frac{H}{H-1}\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{\hat P_i },s\sim \hat P_i(\tilde s,\tilde a)}\braces{f(s,a)}+\frac{1}{H}\EE_{s \sim d_0, a\sim \pi(s_0)}\braces{f(s,a)}. 
\end{align}
The second term in \pref{eq:first}  is upper-bounded by 
\begin{align*}
   \frac{1}{H}\max_{(s,a)}\frac{d_0(s)\pi(a\mid s)}{\rho_i(s,a)}\zeta\leq |\Acal|\zeta 
\end{align*}
Note $\rho(s,a)\geq 1/H d_0(s)u(a\mid s)$ and $\EE_{(s,a)\sim \rho_i}[f(s,a)]\leq \zeta$ with probability $1-\delta$. 

The first term in \pref{eq:first} is further bounded by follows: 
\begin{align*}
    &\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{\hat P_i },s\sim \hat P_i(\tilde s,\tilde a)}\braces{f(s,a)}=\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{\hat P_i }}\hat \phi_i(\tilde s,\tilde a)^{\top}\int \hat \mu_i(s)\pi(a\mid s)f(s,a) d(s,a)\\ 
   &=\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{\hat P_i }} \|\hat \phi_i(\tilde s,\tilde a)\|_{\Sigma_{\rho^{(1)}_i,\hat \phi_i}^{-1}}\|\int \hat \mu_i(s)\pi(a\mid s)f(s,a) d(s,a)\|_{\Sigma_{\rho^{(1)}_i,\hat \phi_i}}.
\end{align*} 
Here, we have 
\begin{align*}
  & \|\int \hat \mu_i(s)\pi(a\mid s)f(s,a) d(s,a)\|^2_{\Sigma_{\rho_i,\hat \phi_i}}\\
&\leq  \braces{\int \hat \mu_i(s)\pi(a\mid s)f(s,a) d(s,a)}^{\top}\braces{i\EE_{(s,a)\sim \rho^{(1)}_i}[\hat \phi \hat \phi^{\top}]+\lambda I  }\braces{\int \hat \mu_i(s)\pi(a\mid s)f(s,a) d(s,a)}\\
&\leq  i \braces{\EE_{(\tilde s,\tilde a)\sim \rho^{(1)}_i}\bracks{\int \hat \mu_i(s)^{\top}\hat \phi_i(\tilde s,\tilde a)\pi(a\mid s)f(s,a) d(s,a)}}^2+ 4\lambda d \\
&=  i \braces{\EE_{(\tilde s,\tilde a)\sim \rho^{(1)}_i, s\sim \hat P_i(\tilde s,\tilde a), a\sim \pi(s)}\bracks{f(s,a) }}^2+ 4\lambda d \\
&\leq  i \braces{\EE_{(\tilde s,\tilde a)\sim \rho^{(1)}_i, s\sim \hat P_i(\tilde s,\tilde a), a\sim \pi(s)}\bracks{f^2(s,a) }}+ 4\lambda d.  \tag{Jensen} 
\end{align*}
Then, 
\begin{align*}
   & i \braces{\EE_{(\tilde s,\tilde a)\sim \rho^{(1)}_i, s\sim \hat P_i(\tilde s,\tilde a), a\sim \pi(s)}\bracks{f^2(s,a) }}+ 4\lambda d \\
  &\leq i \braces{\EE_{(\tilde s,\tilde a)\sim \rho^{(1)}_i, s\sim P^{\star}(\tilde s,\tilde a), a\sim \pi(s)}\bracks{f^2(s,a) }}+ 4\lambda d +i \frac{H}{H-1} \zeta \tag{MLE guarantee}\\
   &\leq \frac{i}{\min\{u(a\mid s)\}}\braces{\EE_{(\tilde s,\tilde a)\sim \rho^{(1)}_i, s\sim P^{\star}(\tilde s,\tilde a), a\sim u(s)}\bracks{f^2(s,a) }}+ 4\lambda d + i  \frac{H}{H-1}\zeta\\
       &= \frac{i}{\min\{u(a\mid s)\}}\braces{\EE_{{\rho}^{(2)}_i}\bracks{f^2(s,a) }}+ 4\lambda d+i \frac{H}{H-1}\zeta\\
                 &\leq \alpha'_i, \alpha'_i=\frac{i|\Acal|}{\gamma}\zeta + 4\lambda d+i \frac{H}{H-1} \zeta.  \tag{MLE guarantee}
\end{align*}
In the end, we have
\begin{align}\label{eq:useful}
\EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\braces{f(s,a)}\leq \sqrt{\alpha'}\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{\hat P_i }} \|\hat \phi_i(\tilde s,\tilde a)\|_{\Sigma_{\rho^{(1)}_i,\hat \phi_i}^{-1}}+\frac{1-\gamma}{\gamma}|\Acal|\zeta. 
\end{align}

Combining all things together,
\begin{align*}
    & \EE_{(s,a)\sim d^{\pi}_{\hat P }}\braces{\EE_{s'\sim \hat P(s,a)}\bracks{V^{\pi}(s') } - \EE_{s'\sim P^{\star}(s,a)}\bracks{V^{\pi}(s') }} \leq H\EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\braces{f(s,a)}\\
   &\leq \frac{ \sqrt{\alpha'}}{1-\gamma}\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{\hat P_i }} \|\hat \phi_i(\tilde s,\tilde a)\|_{\Sigma_{\rho^{(1)}_i,\hat \phi_i}^{-1}}+  \frac{1-\gamma}{\gamma}|\Acal|\zeta.\\
   &\leq \alpha \EE_{(\tilde s,\tilde a)\sim d^{\pi}_{\hat P_i }} \|\hat \phi_i(\tilde s,\tilde a)\|_{\Sigma_{\rho^{(1)}_i,\hat \phi_i}^{-1}}+  \frac{1-\gamma}{\gamma}|\Acal|\zeta,\quad \alpha= \frac{ \sqrt{\alpha'}}{1-\gamma}. 
\end{align*}
   

Going back to the performance different lemma, we have 
\begin{align*}
    V^{\pi}_{\hat P_i,r+\hat b_i}- V^{\pi}&=H\EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\bracks{\hat b(s,a)+\EE_{s'\sim \hat P(s,a)}\bracks{V^{\pi}(s') } - \EE_{s'\sim P^{\star}(s,a)}\bracks{V^{\pi}(s') } }\\
    &\geq H\EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\bracks{ \alpha \|\hat \phi_i (s,a)\|_{\Sigma_{\rho^{(1)}_i,\hat \phi_i}^{-1}}+\EE_{s'\sim \hat P_i(s,a)}\bracks{V^{\pi}(s') } - \EE_{s'\sim P^{\star}(s,a)}\bracks{V^{\pi}(s') } }\\
        &=H\EE_{(s,a)\sim d^{\pi}_{\hat P_i }}\bracks{\alpha\|\hat \phi_i (s,a)\|_{\Sigma_{\rho^{(1)}_i,\hat \phi_i}^{-1}}- \alpha \|\hat \phi_i (s,a)\|_{\Sigma_{\rho^{(1)}_i,\hat \phi_i}^{-1}} }- \frac{1-\gamma}{\gamma}|\Acal|\zeta\\
        &\geq  -\frac{1-\gamma}{\gamma}|\Acal|\zeta.
\end{align*}
\end{proof}

\begin{theorem}
With $1-\delta$, 
\begin{align*}
    &\sum_{k=1}^n \prns{V^{\pi}-V^{\pi_k}}\lesssim \frac{1}{\gamma}|\Acal|\log( |\Fcal|/\delta)+ \sqrt{dn\log(n)}|\Acal|\times \alpha',\\
    &\alpha'=\sqrt{|\Acal|\log( |\Fcal|/\delta)+\alpha^2d+ 4\lambda d+\log( |\Fcal|/\delta)  }.  
\end{align*}
\end{theorem}
(recall $\alpha=O(d)$ since $    \alpha = H\sqrt{\frac{|\Acal|i}{\gamma}\zeta + 4\lambda d+i \zeta},\lambda=O(d)$)
PAC guarantee is obtained by giving a random output from $\pi_1,\cdots,\pi_K$.  The order is roughly $O(d^4|A|^{3}/\epsilon^2)$. 

\masa{can we improve $d$?}

\begin{proof}
Let $Err=|\Acal|/\gamma \zeta$. 
\begin{align*}
        V^{\pi}-V^{\pi_i}& \leq        V^{\pi}_{\hat P_i,r+\hat b_i}-V^{\pi_i}_{P^{\star}}+\mathrm{Err} \tag{Optimism}\\ 
        &\leq       V^{\pi_i}_{\hat P_i,r+\hat b_i}-V^{\pi_i}_{P^{\star}}+\mathrm{Err}\\ 
        &\leq H \EE_{(s,a)\sim d^{\pi_i}_{P^{\star} }}[ \hat b_i(s,a)]+(H)^2 \EE_{(s,a)\sim d^{\pi_i}_{P^{\star} }}[ f(s,a)]+\mathrm{Err}\\
            &\leq H |\Acal|\EE_{(s,a)\sim d^{\pi"_i}_{P^{\star} }}[ \hat b_i(s,a)]+(H)^2|\Acal| \EE_{(s,a)\sim d^{\pi"_i}_{P^{\star} }}[ f(s,a)]+\mathrm{Err}.  
\end{align*}
Here, following \pref{eq:useful}, we have 
\begin{align*}
   \EE_{(s,a)\sim d^{\pi"_i}_{P^{\star} }}[ \hat b_i(s,a)]= \EE_{(\tilde s,\tilde a)\sim d^{\pi"_i}_{P^{\star} }} \|\phi^{\star}(\tilde s,\tilde a)\|_{\Sigma_{\rho_i,\phi^{\star}}^{-1}}\sqrt{\braces{\frac{i|\Acal|}{\gamma}\EE_{\rho^{(1)}_i}\bracks{\hat b^2_i(s,a) }}+ 4\lambda d +i \zeta}+(1-\gamma)\mathrm{Err}.
\end{align*}
In addition, we have 
\begin{align*}
   i\EE_{\rho^{(1)}_i}\bracks{\hat b^2_i(s,a) }=     i \EE_{\rho^{(1)}_i}\bracks{\alpha^2 \|\hat \phi_i(s,a)\|^2_{\Sigma^{-1}_{\rho^{(1)}_i,\hat \phi_i}} }\leq \alpha^2d. 
\end{align*}


Second, following \pref{eq:useful}, we have 
\begin{align*}
   & \EE_{(s,a)\sim d^{\pi"_i}_{P^{\star} }}[ f(s,a)]\\
    &= \EE_{(\tilde s,\tilde a)\sim d^{\pi"_i}_{P^{\star} }} \|\phi^{\star}(\tilde s,\tilde a)\|_{\Sigma_{\rho_i,\phi^{\star}}^{-1}}\sqrt{\braces{\frac{i|\Acal|}{\gamma}\EE_{\rho^{(1)}_i}\bracks{f^2(s,a) }}+4\lambda d+i \zeta}+(1-\gamma)\mathrm{Err}.\\ 
   &\leq \EE_{(\tilde s,\tilde a)\sim d^{\pi"_i}_{P^{\star} }} \|\phi^{\star}(\tilde s,\tilde a)\|_{\Sigma_{\rho_i,\phi^{\star}}^{-1}}\sqrt{\braces{\frac{i|\Acal|}{\gamma}\zeta}+ 4\lambda d+i\zeta}+(1-\gamma)\mathrm{Err}. 
\end{align*}


The first term $\EE_{(\tilde s,\tilde a)\sim d^{\pi"_i}_{P^{\star} }} \|\phi^{\star}(\tilde s,\tilde a)\|_{\Sigma_{\rho_i,\phi^{\star}}^{-1}}$ is upper-bounded as  
\begin{align*}
   &\sum_{i=1}^n \EE_{(\tilde s,\tilde a)\sim d^{\pi"_i}_{P^{\star} }} \|\phi^{\star}(\tilde s,\tilde a)\|_{\Sigma_{\rho_i,\phi^{\star}}^{-1}} \leq \sqrt{n\sum_{i=1}^n \EE_{(\tilde s,\tilde a)\sim d^{\pi"_i}_{P^{\star} }}[\phi^{\star}(\tilde s,\tilde a)^{\top}\Sigma^{-1}_{\rho_i,\phi^{\star}}\phi^{\star}(\tilde s,\tilde a)^{}]} \leq \sqrt{dn\log n}. 
\end{align*}


\end{proof}


\subsection{Auxiliary lemmas}

\begin{lemma}
At episode $i$, with probability $1-\delta$, 
\begin{align*}
  \sum_{j=1}^{i-1} \EE_{(s,a)\sim d^{\pi"_j}}[ \|\hat P_i(\cdot \mid s,a)-P^{\star}(\cdot \mid s,a)\|^2_1 ] \leq i\zeta,\quad \zeta:\coloneqq \ln(|\Psi |\Phi |/\delta)/i.
\end{align*}
The obvious corollary is  with probability $1-\delta$,
\begin{align*}
 \forall i\in N, \sum_{j=1}^{i-1} \EE_{(s,a)\sim d^{\pi"_j}}[ \|\hat P_i(\cdot \mid s,a)-P^{\star}(\cdot \mid s,a)\|^2_1 ] \leq \zeta,\quad \zeta:\coloneqq \ln(|\Psi |\Phi |\log(n)/\delta).
\end{align*}
\end{lemma}



\begin{lemma}\label{lem:con}
Suppose $\lambda=\Omega(d\log(n)\log(|\Phi|))$. With probability $1-\delta$, we have
\begin{align*}
  \forall i,\forall \phi, c_1 \|\phi(s,a)\|_{\Sigma^{-1}_{\rho_i,\phi}}\leq \|\phi(s,a)\|_{\hat \Sigma^{-1}_{i,\phi}} \leq  c_2 \| \phi(s,a)\|_{\Sigma^{-1}_{\rho_i,\phi}}. 
\end{align*}
\end{lemma}




---------------------

not changed yet 

-------------------------

\begin{lemma}\label{lem:useful}
Define $\Sigma_{\rho,\phi^{\star}}=n\EE[\phi^{\star}\{\phi^{\star}\}^{\top}]+\lambda I$. Then, 
{\small 
\begin{align*}
    \EE_{(s,a)\sim d^{\pi}_{P^{\star} }}\braces{f(s,a)}\leq \EE_{(\tilde s,\tilde a)\sim d^{\pi}_{P^{\star} }} \|\phi^{\star}(\tilde s,\tilde a)\|_{\Sigma_{\rho,\phi{\star}}^{-1}}\sqrt{ \frac{n}{\min\{\pi_b(a\mid s)\}}\braces{\frac{1}{\gamma}\EE_{\rho}\bracks{f^2(s,a) }}+ 4\lambda d+i\zeta}+(1-\gamma) \max_{(s,a)}\frac{d_0(s)\pi(a\mid s)}{\rho(s,a)}\zeta. 
\end{align*}
}
\end{lemma}
\begin{proof}
Besides, by the one-step-back trick,
\begin{align}\label{eq:first_true}
    \EE_{(s,a)\sim d^{\pi}_{P^{\star} }}\braces{f(s,a)}=\gamma   \EE_{(\tilde s,\tilde a)\sim d^{\pi}_{P^{\star} },s\sim P^{\star}(\tilde s,\tilde a),a\sim \pi(s)}\braces{f(s,a)}+(1-\gamma)\EE_{s \sim d_0, a\sim \pi(s_0)}\braces{f(s,a)}. 
\end{align}
The second term in \pref{eq:first_true}  is upper-bounded by 
\begin{align*}
   (1-\gamma) \max_{(s,a)}\frac{d_0(s)\pi(a\mid s)}{\rho(s,a)}\zeta. 
\end{align*}


The first term in \pref{eq:first_true} is further bounded by follows: 
\begin{align*}
    &\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{P^{\star} },s\sim P^{\star}(\tilde s,\tilde a),a\sim \pi(s)}\braces{f(s,a)}=\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{P^{\star} }}\phi^{\star}(\tilde s,\tilde a)^{\top}\int \mu^{\star}(s)\pi(a\mid s)f(s,a) d(s,a)\\ 
   &=\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{P^{\star} }} \|\phi^{\star}(\tilde s,\tilde a)\|_{\Sigma_{\rho, \phi^{\star}}^{-1}}\|\int \mu^{\star}(s)\pi(a\mid s)f(s,a) d(s,a)\|_{\Sigma_{\rho,\phi^{\star}}}.
\end{align*} 

Here, we have 
\begin{align*}
  & \|\int \mu^{\star}(s)\pi(a\mid s)f(s,a) d(s,a)\|^2_{\Sigma_{\rho,\phi^{\star}}}\\
&\leq  \braces{\int  \mu^{\star}(s)\pi(a\mid s)f(s,a) d(s,a)}^{\top}\braces{n\EE_{(s,a)\sim \rho}[\phi^{\star}(s,a) \{\phi^{\star}(s,a)\}^{\top} ]+\lambda I  }\braces{\int \mu^{\star}(s)\pi(a\mid s)f(s,a) d(s,a)}\\
&\leq  n \braces{\EE_{(\tilde s,\tilde a)\sim \rho}\bracks{\int \mu^{\star}(s)^{\top}\phi^{\star}(\tilde s,\tilde a)\pi(a\mid s)f(s,a) d(s,a)}}^2+ 4\lambda d \\
&=  n \braces{\EE_{(\tilde s,\tilde a)\sim \rho, s\sim P^{\star}(\tilde s,\tilde a), a\sim \pi(s)}\bracks{f(s,a) }}^2+ 4\lambda d \\
&\leq  n \braces{\EE_{(\tilde s,\tilde a)\sim \rho, s\sim P^{\star}(\tilde s,\tilde a), a\sim \pi(s)}\bracks{f^2(s,a) }}+ 4\lambda d.  \tag{Jensen} 
\end{align*}
Then, 
\begin{align*}
  & n \braces{\EE_{(\tilde s,\tilde a)\sim \rho, s\sim P^{\star}(\tilde s,\tilde a), a\sim \pi(s)}\bracks{f^2(s,a) }}+ 4\lambda d +n \zeta \\
   &\leq \frac{n}{\min\{\pi_b(a\mid s)\}}\braces{\EE_{(\tilde s,\tilde a)\sim \rho, s\sim P^{\star}(\tilde s,\tilde a), a\sim \pi_b(s)}\bracks{f^2(s,a) }}+ 4\lambda d + n \zeta\\
       &= \frac{n}{\min\{\pi_b(a\mid s)\}}\braces{\frac{1}{\gamma}\EE_{\rho}\bracks{f^2(s,a) }-\frac{1-\gamma}{\gamma}\EE_{s\sim d_0,a\sim \pi_b(s)}\bracks{f^2(s,a) }}+ 4\lambda d+i\zeta\\
         &\leq \frac{n}{\min\{\pi_b(a\mid s)\}}\braces{\frac{1}{\gamma}\EE_{\rho}\bracks{f^2(s,a) }}+ 4\lambda d+i\zeta\\
                 &\leq \alpha', \alpha'=\frac{n}{\gamma \min\{\pi_b(a\mid s)\}}\zeta + 4\lambda d+n \zeta. 
\end{align*}
In the end, we have
\begin{align}\label{eq:useful}
\EE_{(s,a)\sim d^{\pi}_{P^{\star} }}\braces{f(s,a)}\leq \sqrt{\alpha'}\EE_{(\tilde s,\tilde a)\sim d^{\pi}_{P^{\star} }} \| \phi^{\star}(\tilde s,\tilde a)\|_{\Sigma_{\rho,\phi^{\star}}^{-1}}+(1-\gamma) \max_{(s,a)}\frac{d_0(s)\pi(a\mid s)}{\rho(s,a)}\zeta. 
\end{align}

\end{proof}

\begin{lemma}[Agnostic Generalization error of linear regression]
Let $\{(x_i,y_i)\}_{1:n}$ be generated as $x_i\sim\rho$, $\EE[y_i|x_i] = f(x_i)$, $|y|\leq H$. We have
\begin{equation}
    \EE_{x\sim\rho}\left[(E[y|x]-\hat\theta^\top x)^2\right]\leq O\left(\frac{H^2d\log(1/\delta)}{n}\right)+\frac{1}{n}\sum_{i=1}^n \left((\tilde \theta^\top x_i-y_i)^2-(f(x_i)-y_i)^2\right)
\end{equation}
where $\tilde\theta = \min_\theta \EE_{x\sim\rho}[(y-\theta^\top x)^2]$.

\end{lemma}


